A Survey of Microarchitectural Side-channel Vulnerabilities, Attacks and Defenses in Cryptography

Side-channel attacks have become a severe threat to the confidentiality of computer applications and systems. One popular type of such attacks is the microarchitectural attack, where the adversary exploits the hardware features to break the protection enforced by the operating system and steal the secrets from the program. In this paper, we systematize microarchitectural side channels with a focus on attacks and defenses in cryptographic applications. We make three contributions. (1) We survey past research literature to categorize microarchitectural side-channel attacks. Since these are hardware attacks targeting software, we summarize the vulnerable implementations in software, as well as flawed designs in hardware. (2) We identify common strategies to mitigate microarchitectural attacks, from the application, OS and hardware levels. (3) We conduct a large-scale evaluation on popular cryptographic applications in the real world, and analyze the severity, practicality and impact of side-channel vulnerabilities. This survey is expected to inspire side-channel research community to discover new attacks, and more importantly, propose new defense solutions against them.

==> tex/lesson.tex <==
\section{Insights and Lessons}
\label{sec:lesson}

We draw some insights and suggestions based on the summarization and 
evaluation of side-channel vulnerabilities and countermeasures. We hope they can benefit 
cryptographic software developers, users and researchers.

\subsection{Research Directions}
First, we propose several promising opportunities and directions for future side-channel research. 

\bheading{D1: Identify new vulnerabilities in state-of-the-art cryptographic implementations, more likely in less-studied ciphers and operations.}

%Are there new vulnerabilities in current cryptographic implementations? Are there other ciphers or operations containing side-channel vulnerabilities?

The discovery and exploitation of various side-channel vulnerabilities during the past decades
inspired people to search for new secure solutions. Now each critical cryptographic primitive
has secure algorithms and implementations that are robust against different types of side-channel attacks. 
%New vulnerabilities reported by recent papers are mainly due to small accidental software bugs, and can be easily fixed. 
Thus, it is interesting
to explore new fundamental vulnerabilities in current implementations. In addition to the cryptographic
operations discussed in \secref{sec:crypto}, researchers can focus on other ciphers and operations, and
search for new critical vulnerabilities.
For instance, the emerging post-quantum cryptography has drawn people's attention for its resistance against quantum computer based attacks. Different types of
post-quantum algorithms were designed for public key infrastructure, e.g., hash-based, lattice-based and multivariate cryptography. Currently researchers only focus on the
side-channel vulnerabilities in lattice-based cryptography. It is interesting to explore
if there are any chances to attack other types of post-quantum cryptography schemes. 

\bheading{D2: Discover outdated vulnerabilities in less popular and closed-source
applications.}

As discussed in \secref{sec:cross-library-comp}, old vulnerabilities, especially those against cryptographic primitives or 
via micro-architectural contention, can still exist in real-world applications. It is worth the research effort to conduct a more
comprehensive evaluation of various side-channel vulnerabilities on different open-source 
libraries and commercial products. This will raise public awareness on side-channel threats, 
and more importantly, encourage developers to secure these applications as a result.


\bheading{D3: Design new side-channel attack techniques that can capture finer grained side-channel information, and study countermeasures for the new attacks.}

From \secref{sec:crypto} we observe that innovation in providing adversaries with more detailed information
usually exposes new vulnerabilities. For instance, fixed window modular exponentiation with 
scatter-gather approach was designed to defeat attacks with 
the granularity of cache line. However, a new attack method that 
captures cache-bank level information \cite{YaGeHe:17} invalidated the approach. Previous 
countermeasures for padding oracle attacks only considered remote attacks, and thus they
focused on producing uniform responses in constant time. Later, host-based attack techniques
were applied to padding oracle settings \cite{RoGiGe:19, IrLnEi:15, XiLiCh:17, RoPaSh:18},
compromising such solutions. We hence propose this research direction so
the security of cryptographic operations can be constantly enhanced. 



\subsection{Development Recommendations}
We offer some suggestions for developers of cryptographic applications and systems to make
the implementations more secure and efficient.

\bheading{R1: Different countermeasure strategies can have different vulnerability coverages
and performance costs. Developers need to carefully select the optimal strategies for critical
operations.}

We summarized different countermeasures and their features in \secref{sec:insights}. 
To remove control flow vulnerabilities, AlwaysExecute strategies introduce performance 
overhead due to execution of all possible code routines. ConditionalSelect can only defeat 
remote attacks since it still leaves a minor secret-dependent control flow, while 
BitwiseSelect is secure against all known types of attacks.

To remove data flow vulnerabilities, AlwaysAccess-BitwiseSelect defeats all known types of 
attacks with the price of performance degradation from extra memory accesses. On-the-fly 
calculation is useful if the computation does not contain secret-dependent control flows, while repeated computation causes slowdown.

Cryptographic blinding is a technique dedicated for asymmetric cryptography such as RSA, ElGamal and ECC.
It is particularly effective in cases where secret-dependent control flow or data flow 
is hard to remove (e.g., modular multiplication).
Plaintext/ciphertext blinding can only defeat chosen-input side-channel attacks, while key 
blinding does not have this limitation.

\bheading{R2: Software bugs contribute a lot to side-channel vulnerabilities.
Developers should verify the code correctness of critical operations prior to release.}

Developers may accidentally leave software bugs that can be exploited to perform
side-channel attacks. As critical cryptographic operations are designed to be more
secure today, adversaries now tend to search such bugs to break the secure
designs and implementations (\secref{sec:count-type}). There are three common types of 
side-channel bugs. 
First, incorrect flag propagation prevents some cryptographic
operations from calling the securely implemented routine even though it is already introduced,
exemplified by modular exponentiation \cite{GaBrYa:16} and inversion
\cite{GaPeBr:16}. Second, some secure implementations are only partly applied to the
operations or primitives, leaving the rest still vulnerable. 
For instance, in OpenSSL before version 1.0.2q, most curves (P-224, P-256 and P-521) adopted
secure branchless Montgomery ladder or masked window for scalar multiplication,
but P-384 curve still used the insecure sliding window implementation, offering the adversary
an opportunity to compromise ECDSA \cite{AlBrHa:19}. Third, some corner cases were overlooked
during implementation, giving rise to non-constant runtime behaviors in execution time
\cite{AlPa:16, RoPaSh:18}, message type \cite{MeSoJu:14} and format \cite{AvScSo:16}.

\iffalse
Generally, software bugs that can lead to side-channel vulnerabilities can be classified
into two categories. First, selection of secure code routine.
Some libraries provide both secure and insecure implementations for one cryptographic
operation. One type of software bugs is that the operation fails to call the secure
implementation routine. There are multiple reasons: (1) implementation selection is 
determined by a flag. However, the propagation of this flag can contain software bugs
that even the secure implementation flag is specified at the beginning, it may not be
properly passed to the caller function and the insecure implementation is still called. 
This happened in the modular exponentiation \cite{GaBrYa:16} and modular inverse
\cite{GaPeBr:16} functions. (2) Some secure implementations are not default options, and
require users to add extra compiler flags to enable them. If users are not aware of these
features and still use the default options, then their applications are still vulnerable.
For instance, the secure masked-window scalar multiplication was introduced in OpenSSL
1.0.1. After that, there are still attacks \cite{BeVaSm:14, VaSmYa:15, GePaPi:16, FaWaCh:16,
AlBrFa:16} proposed against scalar multiplication in OpenSSL after version 1.0.1,
as they compiled the library using the default option with the vulnerable $w$-ary NAF
implementation. (3) Some secure implementations were introduced and applied to part of
the operations or primitives, leaving the rest still vulnerable. For instance, 
ECC offers many curves for cryptographic operations. In OpenSSL before version 1.0.2q,
most curves (P-224, P-256 and P-521) adopted secure branchless montgomery ladder or
masked-window implementations for scalar multiplication. However, P-384 curve still used
the insecure $w$-ary NAF implementation. This gave the adversary an opportunity to
compromise ECDSA \cite{AlBrHa:19}.

Second, unexpected inconstant behaviors. Some implementations in cryptographic protocols
try to remove side channels by providing constant outputs independent of the inputs.
However, some corner cases were missed, which could give inconstant function counts or
timing \cite{AlPa:16}, non-uniform message types \cite{MeSoJu:14} or formats
\cite{AvScSo:16}. These can be exploited by the adversary as side channels to compromise the 
protocols.
\fi

To verify if the secure routines are selected properly and applied to all operations or 
primitives, developers can insert
breakpoints inside the insecure routines and check if they are reached \cite{AlGaTa:18}.
To verify if the implementation has expected constant behaviors, developers can measure
the side-channel information under different cases and check if they are indistinguishable.


\bheading{R3: Developers should carefully handle the reported vulnerabilities. They should (1) prioritize the most severe vulnerabilities; (2) apply patches to all live
branches at the same time; (3) apply patches to all vulnerable operations.}

From \secref{sec:vul-severe} we observe that different types of side-channel vulnerabilities
are assigned with different severity scores. The network-level vulnerabilities are 
particularly severe as they are more exploitable, so developers should pay special attention 
to those attacks and prioritize their fixes. Besides, when a vulnerability is 
disclosed, developers should apply the corresponding countermeasure patches to all live 
branches of the application immediately. Otherwise, the unpatched branch will remain 
vulnerable as the threat is disclosed to the public (\secref{sec:cross-branch}). Developers 
should also check whether the application contains other implementations sharing the 
same vulnerability. If so they should also fix them even though they are not reported. 

\subsection{Indications in Practice}
We draw some conclusions for cryptographic application users about side-channel threats and
countermeasures from a practical viewpoint.

\bheading{I1: Side-channel vulnerabilities are generally considered less severe compared to
other vulnerabilities, although their volume in CVE database is non-trivial.}

As discussed in \secref{sec:vul-severe}, two reasons make side-channel threats less severe:
the attacks require higher adversarial capabilities and more domain knowledge,
and the damage is relatively smaller. Thus, the existence of these vulnerabilities in 
applications is by no means a catastrophe to the users and there is no need to panic.
The world has not seen an occurrence of malicious side-channel attacks that could bring severe damages so far.

\bheading{I2: Although side-channel vulnerabilities are regarded as less severe, they are handled
very actively, either in mainstream open-source libraries (\secref{sec:vul-resp}), less
popular libraries or closed-source products (\secref{sec:cross-library-comp}).}

Such active attitude towards side-channel threats is reflected in several aspects. First, new
side-channel vulnerabilities were fixed at a very fast speed to reduce users' potential damage.
Second, most known side-channel vulnerabilities to date were fixed. Third, cryptographic libraries
are now shifting the countermeasures from brand new implementations to minor bug fixes and
enhancement, indicating that they are becoming more mature (\secref{sec:count-type}).

\bheading{I3: It is unnecessary for users to always patch or upgrade the libraries for the most
secure implementations. They can adopt those suited to their scenarios.}

If a use case does not need to consider certain adversarial capabilities, countermeasures designed
for them will not be necessary. For instance, if the application does not have network interfaces,
then the user does not need to consider network-level side-channels. If the application does not
share the computing platform with other untrusted parties, then the user does not need to consider
host-level attacks.



